Adaptive Gaussian process surrogates for Bayesian inference

We present an adaptive approach to the construction of Gaussian process surrogates for Bayesian inference with expensive-to-evaluate forward models. Our method relies on the fully Bayesian approach to training Gaussian process models and utilizes the expected improvement idea from Bayesian global optimization. We adaptively construct training designs by maximizing the expected improvement in fit of the Gaussian process model to the noisy observational data. Numerical experiments on model problems with synthetic data demonstrate the effectiveness of the obtained adaptive designs compared to the fixed non-adaptive designs in terms of accurate posterior estimation at a fraction of the cost of inference with forward models.

==> posterior.tex <==
%!TEX root = mainAdaptiveGP.tex

%% COPIED OVER TO IMPLEMENTATION

\section{Posterior estimation}

In the following numerical examples the estimation of the posterior is performed with emcee \cite{DForemanMackey_DWHogg_DLang_JGoodman_2013a}. It requires providing the log-probability function that is a product of the log-prior and log-likelihood.
For the ``true'' likelihood $L(\theta | \bz)$ the log-likelihood is (assuming diagonal noise covariance $\BSigma_{E}$) is computed as follows:
\[
	\log L(\theta | \bz) = -\frac{1}{2} \sum_{i=1}^q \bigg[ \frac{(z_i - f_i(\theta))^2}{2\pi \sigma_i^2} + \log(2\pi \sigma_i^2) \bigg].
\]
For the GP-based likelihood $L(\theta | \bz, \cD)$ the log-likelihood is approximated as:
\[
	\log L(\theta | \bz, \cD) \approx \log\bigg( \sum_{j=1}^{n_\psi} \frac{k^{(j)}}{n_\psi} \exp\left[-\frac{1}{2} g\big(\theta; \cD, \psi^{(j)}\big) \right] \bigg).
\]
In order to avoid underflow when computing this approximation we use the following LogSumExp formulation:
\[
	\log L(\theta | \bz, \cD) \approx -\frac{1}{2}g^* + \log\bigg( \sum_{j=1}^{n_\psi} \frac{k^{(j)}}{n_\psi} \exp\left[-\frac{1}{2} \big(g\big(\theta; \cD, \psi^{(j)}\big) - g^*\big) \right] \bigg),
\]
where
\[
	g^* =\min_j g\big(\theta; \cD, \psi^{(j)}\big).
\]
